A Phenomenological Analysis of LHC Neutrino Scattering at NLO Accuracy Matched to Parton Showers

We perform a detailed phenomenological study of high-energy neutrino deep inelastic scattering (DIS) focused on LHC far-forward experiments such as FASER$\nu$ and SND@LHC. To this aim, we parametrise the neutrino fluxes reaching these LHC far-forward experiments in terms of `neutrino PDFs' encoding their energy and rapidity dependence by means of the LHAPDF framework. We integrate these neutrino PDFs in the recently developed POWHEG-BOX-RES implementation of neutrino-induced DIS to produce predictions accurate at next-to-leading order (NLO) in the QCD coupling matched to parton showers (PS) with Pythia8. We present NLO+PS predictions for final-state distributions within the acceptance of FASER$\nu$ and SND@LHC as well as for two experiments of the proposed Forward Physics Facility (FPF), FASER$\nu$2 and FLArE. We quantify the impact of NLO QCD corrections, of the parton showering and hadronisation settings in Pythia8, of the QED shower, and of the incoming neutrino flavour for the description of these observables, and compare our predictions with the GENIE neutrino event generator. Our work demonstrates the relevance of modern higher-order event generators to achieve the key scientific targets of the LHC neutrino experiments.

==> tables/detectors.tex <==
%-----------------------------------------------------------------
\begin{table}[t]
  \centering
  \small
  \renewcommand{\arraystretch}{1.50}
\begin{tabularx}{\textwidth}{Xccccc}
\toprule
Detector &  Rapidity &  Target & Charge ID & Acceptance  & Performance \\
\midrule
\midrule
\multirow{3}{*}{FASER$\nu$}  &  \multirow{3}{*}{ $\eta_\nu \ge 8.5$}  &   \multirow{2}{*}{Tungsten}  & \multirow{3}{*}{muons}      &   $E_\ell,E_h \gsim 100$ GeV   &      $\delta E_\ell \sim 30\% $    \\
&   &   \multirow{2}{*}{(1.1 ton)}  &       &  $\tan \theta_\ell \lsim 0.025$   &
$\delta \theta_\ell \sim 0.06$ mrad        \\
&   &     &       &  reco $E_h$ \& charm ID   &      $\delta E_h \sim 30\%$     \\
\midrule
\multirow{2}{*}{SND@LHC}  & \multirow{2}{*}{ $7.2 \le \eta_\nu \le 8.4$}   &  Tungsten   &   \multirow{2}{*}{n/a}    &  $E_\ell,E_h \gsim 20 $ GeV     &    \multirow{2}{*}{n/a}    \\
  &    &  (0.83 ton)   &  &  $\theta_\mu \lsim 0.15, \theta_e \lsim 0.5$         &       \\
\midrule
\midrule
\multirow{3}{*}{FASER$\nu$2}  & \multirow{3}{*}{ $\eta_\nu \ge 8.5$}  & \multirow{2}{*}{Tungsten}    &   \multirow{3}{*}{muons}     &   $E_\ell,E_h \gsim 100$ GeV  &    $\delta E_\ell \sim 30\% $     \\
  &   &  \multirow{2}{*}{(20 ton)}   &       &  $\tan \theta_\ell \lsim 0.05$   &   $\delta \theta_\ell \sim 0.06$ mrad      \\
  &   &     &       &  reco $E_h$ \& charm ID   &  $\delta E_h \sim 30\%$        \\
\midrule
\multirow{3}{*}{AdvSND-far}  &   \multirow{3}{*}{ $7.2 \le \eta_\nu \le 8.4$}  &
\multirow{2}{*}{Tungsten}   &   \multirow{3}{*}{muons}    &  $E_\ell,E_h \gsim 20 $ GeV  & \multirow{3}{*}{n/a}          \\
  &   &   \multirow{2}{*}{(5 ton)}  &        & $\theta_\mu \lsim 0.15, \theta_e \lsim 0.5$     &           \\
  &   &     &       &  reco $E_h$   &           \\
\midrule
\multirow{3}{*}{FLArE ({\bf *})}  & \multirow{3}{*}{$\eta_\nu \ge 7.5$} & \multirow{2}{*}{LAr}  & \multirow{3}{*}{muons}  &  $E_\ell,E_h \gsim 2$ GeV, $E_e \lsim 2$ TeV    &    $\delta E_e \sim 5\% $,  $\delta E_\mu \sim 30\% $ \\
&   &  \multirow{2}{*}{(10,~100~ton)}   &   & $\theta_\mu \lsim 0.025$, $\theta_e \lsim 0.5$ &    $\delta \theta_\ell \sim 15 $ mrad\\
 &   &     &  & reco $E_h$  &    $\delta E_h \sim 30\% $   \\
  \bottomrule
\end{tabularx}
\vspace{0.2cm}
\caption{\small For each of the far-forward LHC neutrino experiments considered,
   we indicate their neutrino pseudo-rapidity coverage, target material, whether
  they can identify the sign of the outgoing charged lepton,
  the acceptance for the charged lepton and hadronic final state,
  and the expected reconstruction performance.
  %
  We consider separately acceptance and performance for electron and muon
  neutrinos.
  %
  For FLArE, we assume that muons would be measured in the FASER2 spectrometer
  situated downstream in the FPF cavern.
  %
  See the description of each experiment in the text for more details.
  %
  For our projections we assume that FASER$\nu$ and SND@LHC acquire data
  for the Run III period ($\mathcal{L}=150$ fb$^{-1}$), while FASER$\nu$2, AdvSND, and FLArE take data
  for the complete HL-LHC period ($\mathcal{L}=3$ ab$^{-1}$).
  %
  In the case of FLArE, we consider results both
  for 10 ton and 100 ton fiducial volume detectors.
  \label{tab:FPF_experiments}
}
\end{table}
%-----------------------------------------------------------------


==> tables/integrated_yields.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------------------------------
\begin{table}[t]
  \centering
  \small
  \renewcommand{\arraystretch}{1.70}
\begin{tabularx}{\textwidth}{X||c|c|c||c|c|c}
\toprule
Detector & $\quad$ $N_{\nu_e}$ $\quad$ &$\quad$ $N_{\bar{\nu}_e}$$\quad$   &   $N_{\nu_e} + N_{\bar{\nu}_e}$ &
$\quad$$N_{\nu_\mu}$ $\quad$ & $\quad$ $N_{\bar{\nu}_\mu}$ $\quad$  &   $N_{\nu_\mu} + N_{\bar{\nu}_\mu}$ \\
\midrule
\midrule
FASER$\nu$  & 0.2k (31)    & 110 (19)  & 0.3k (50)  &  0.6k (98)  &  0.3k (45)  &  0.9k (140) \\
SND@LHC  &  88 (11)  & 38 (5.4)    & 130 (16)   &  0.3k (54) & 96 (22)   &  0.4k  (76)\\
\midrule
\midrule
FASER$\nu$2  & 58k (8.3k)   & 28k (5.0k)   & 86k (13.3k)  & 190k (27k)  & 67k (12k)    & 260k (39k)   \\
AdvSND-far  &  5.9k (0.7k)  & 2.8k (0.4k)   & 8.7k (1.1k)  & 20k (2.4k)  & 8k (1.1k)   & 28k (3.5k)   \\
FLArE10 & 22k (2.7k) & 10k (1.5k)   &  32k (4.2k) &  38k (5.2k)&   19k (2.5k) &   57k (7.7k) \\
FLArE100 &   140k (18k)         &    66k (9.5k)         &       210k (27k)       &   220k (30k)      &  120k (15k)    &  340k (45k)  \\
  \bottomrule
\end{tabularx}
\vspace{0.2cm}
\caption{\small Integrated event yields for the six detectors considered,
  separated into electron neutrinos and antineutrinos,
  muon neutrinos and antineutrinos, and their sum.
  %
  These event yields are computed from Eq.~(\ref{eq:event_yields_calculation})
  imposing DIS kinematics, $Q^2 \ge 2$ GeV$^2$ and $W^2 \ge 4$ GeV$^2$.
  %
 The numbers in parenthesis indicate the event rates corresponding to charm
 production.
 %
 In the case of the FLArE detector, we display results for two proposed
 options with fiducual masses of 10 and 100 tons respectively.
  \label{tab:integrated_rates}
}
\end{table}
%-----------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

